PIVOT: Preference-based Intervention Vectors for Pedagogical Tutor Steering

LLMs are increasingly used for conversational tutoring, but effective tutoring requires more than correct answers. Tutors must choose when to scaffold reasoning, hint, give feedback, explain, or invite reflection. Existing prompting and training methods improve pedagogical alignment, but lack reliable inference-time control over pedagogical strategies. We introduce PIVOT, an activation-steering framework that learns preference-based intervention vectors online for frozen LLM tutors. PIVOT uses a seven-category tutor-move taxonomy and a generate-label-optimise loop, where a human-validated LLM judge identifies target and confusable non-target moves to construct preference pairs for multi-layer residual-stream steering. Across held-out and out-of-domain tutoring data, PIVOT controls tutor moves while preserving relevance and fluency, and its directions can be scaled, transferred, and composed at inference time. In a user study with 30 teachers, 73.3% of participants preferred steered conversations over neutral baseline interactions using the same prompt, and rated the controls as clear, usable, and pedagogically meaningful.

==> sections/appendices/prompt_alpha_eval.tex <==
\section{Prompt Alpha Eval}
\label{appen:prompt-alpha}

==> sections/introduction_v1.tex <==

% LLMs have been used in education
% one thing is tutoring and very effective
% Personalised learning, tutoring needs to be controllable 
% However, LLMs halucinate, and hard to control
% One way is to Prompt, tool calling, finetuning or even RL 
% THERE IS THE ISSUE OF COMMON MOVES RUBRIC NO ONE MADE IT YET
% Another way that has become popular is activation steering
% Activation steering has been succeful in behavioural: General activation steering, CAA, BiPO,..
% But:
% 1- tutoring is not that one direction and its opposite, it's multidirectional there is no absolute negative and may not live in one layer as this paper says
% 2- We don't have a dataset with clear and unified tutor moves
% So what do we do:
% 1- We create a rubric: we borrow from the OG autotutor, and we combine it with metacognitive, feedback and funneling to create a comprehensive tutoring moves rubric
% 2- We introduce self-discovery Preperece training method with automatic weighting for tutoring moves to get the model to disover and build 
% Our results show that we steer this amount and it generalises on unseen data
% we run a user study that shows ......
% Our contributions are as follows

\section{Introduction}

Large language models (LLMs) are increasingly being developed and evaluated for personalised educational applications \cite{jurenka2025responsibledevelopmentgenerativeai}. LLMs have been applied to wide range of educational tasks including question generation \cite{scaria2024automated,2024_Hang}, automatic feedback generation \cite{fawzi2026refinerealworldexplorationinteractive, 10.1007/978-3-031-72315-5_20} interactive explanation \cite{fawzi-etal-2025-scribe}, and conversational tutoring \cite{sonkar-etal-2023-class,NEURIPS2024_9bae399d,dinucu-jianu-etal-2025-problem}.

Conversational tutoring is a promising educational application of LLMs because it can provide scalable, individualised support to learners \cite{jurenka2025responsibledevelopmentgenerativeai,puech-etal-2025-towards}. However, effective tutoring requires more than producing correct answers. Real-time tutoring requires models to identify student errors, select appropriate pedagogical strategies, and guide students towards constructing solutions rather than directly receiving them, since productive challenges can support more durable learning than immediate answer provision \cite{maurya-etal-2025-unifying,dinucu-jianu-etal-2025-problem,bjork2011making}. This goal is difficult for LLMs because they are typically optimised for assistant-like helpfulness rather than pedagogical behaviour \cite{puech-etal-2025-towards,sonkar-etal-2024-pedagogical}. As a result, LLM tutors may reveal answers too early, provide too much support, or fail to sustain productive multi-turn tutoring interactions \cite{puech-etal-2025-towards,zhao2026evaluatinganswerleakagerobustness}.

% Teaser figure
\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{figures/pull_figure.pdf}
    \caption{}
    \label{fig:pull}
\end{figure}

Prior work improves LLM tutor alignment by prompting models to follow explicit pedagogical decisions, including step-by-step scaffolding \cite{sonkar-etal-2023-class}, adaptation to student states \cite{10.1145/3613905.3651122}, course-plan updates from interaction history \cite{10.1145/3627673.3679665}, and strategy-level steering through student-state transitions \cite{puech-etal-2025-towards}. Other work uses supervised fine-tuning on human or synthetic tutoring dialogues to embed pedagogical behaviour in the model \cite{jurenka2025responsibledevelopmentgenerativeai,macina-etal-2023-mathdial,sonkar-etal-2023-class}. Recent methods further optimise tutors with Direct Preference Optimisation (DPO) \cite{rafailov2023direct} or reinforcement learning from simulated student-tutor interactions \cite{10.1007/978-3-031-98414-3_18,dinucu-jianu-etal-2025-problem}. While these approaches improve pedagogical alignment, they still leave tutor moves difficult to control at inference time. Prompting can break across contexts or adversarial student requests \cite{puech-etal-2025-towards,zhao2026evaluatinganswerleakagerobustness}. Training-based methods bake behaviours into model parameters rather than expose per-response control \cite{10.1007/978-3-031-98414-3_18,dinucu-etal-2025-problem}. Similar to prompt-only approaches, this alignment can still break under adversarial student behaviour \cite{zhao2026evaluatinganswerleakagerobustness}. 

Activation steering offers a promising alternative to prompting and training-based alignment because it can modulate behaviour at inference time without adding prompt instructions or updating model weights \cite{rimsky-etal-2024-steering,cao2024personalized,10.5555/3737916.3742333}. Activation Addition builds steering vectors from activation differences between contrastive pairs, such as desired versus undesired responses to the same input \cite{turner2024steering}. Contrastive Activation Addition extends this by averaging residual-stream activation differences over many contrastive pairs, enabling control over traits such as sycophancy and hallucination while largely preserving capabilities \cite{rimsky-etal-2024-steering}. BiPO further optimises these vectors with preference pairs in a DPO-style objective, improving control for truthfulness, hallucination mitigation, and jailbreak defence \cite{cao2024personalized}. In tutoring, recent work adapts this idea to steer tutor-specific behaviour and style from human tutor-student dialogues, but not explicit pedagogical moves \cite{lee2026lettingtutorpersonasspeak}. Extending activation steering from broad tutor style to pedagogical moves therefore requires defining both the move categories and the contrasts used to steer them.

Prior work shows that tutoring behaviour can be decomposed into distinct dialogue moves. Early tutoring systems such as AutoTutor define moves for eliciting, guiding, correcting, and explaining student reasoning \cite{Graesser2004}. Classroom discourse work studies how teachers guide student thinking through questioning and talk moves \cite{herbel2005questioning,hagenah2018funneling,alic-etal-2022-computationally,OCONNOR2019166}. Human-human tutoring dialogue mining identifies strategies such as probing, hinting, and feedback \cite{LIN2022194}, while \cite{macina-etal-2023-mathdial} defines math-tutoring moves such as focus, probing, and telling for LLM-based tutoring data collection. However, these taxonomies are designed for different settings and levels of analysis, and do not provide a unified set of tutor moves for activation steering. Moreover, tutor moves are not naturally binary opposites in the way safety steering can contrast safe and unsafe generations, making contrast construction less direct.

In this work, we introduce PIVOT, a framework for preference-based intervention vectors that enables inference-time control over pedagogical tutor moves in frozen LLMs. We derive a tutor-move taxonomy from prior work across tutoring systems, classroom discourse, human-human tutoring, and LLM-based tutoring. Since there are no unified labels or clean contrastive data for steering, PIVOT learns contrasts online with a human-validated LLM judge that identifies target and confusable non-target moves. These pairs optimise multi-layer residual-stream steering vectors with a DPO objective, enabling moves to be activated, scaled, and combined at inference time without updating model weights. Figure~\ref{fig:pull} shows that PIVOT can steer the same tutoring context toward different pedagogical moves while preserving relevance. Our evaluation combines automatic assessment with the human-validated judge and a teacher user study. PIVOT improves target-move control while preserving relevance and fluency, transfers to tutoring data unseen during training, and is preferred by 73.3\% of teachers over a neutral tutor conversation. Our main contributions are:

\begin{enumerate}
    \item We introduce PIVOT, a framework for inference-time tutor-move control using preference-based, multi-layer residual-stream steering vectors.
    \item We derive a tutor-move taxonomy for controllable LLM tutoring by combining prior work across tutoring systems, classroom discourse, human-human tutoring, and LLM-based tutoring.
    \item We propose an online preference construction method that uses a human-validated LLM judge to identify target and confusable non-target tutor moves for DPO-style steering-vector optimisation.
    \item We evaluate PIVOT across validation, held-out, and tutoring data unseen during training, including steering-strength sensitivity and layer ablations.
    \item We conduct a teacher user study showing that controllable tutor moves improve perceived pedagogical control and are preferred over neutral tutor generation.
\end{enumerate}

% Two challenges remain. First, there is no unified operational rubric for steering LLMs across fine-grained tutoring moves. Prior tutoring research provides rich taxonomies, including AutoTutor-style dialogue acts, feedback, funnelling, focusing, and metacognitive support, but these categories are not packaged as a practical control interface for modern LLM tutors. Second, tutoring moves do not fit the binary contrast structure assumed by many steering methods: a hint is not simply the negative of feedback, and metacognitive reflection is not the opposite of assertion.





% Activation steering offers a lightweight alternative by adding learned or extracted vectors to internal model activations at inference time. Methods such as activation addition, CAA, and BiPO show that steering vectors can shift generations toward desired behaviours without updating model weights. Yet tutor-move steering is multi-directional, context-dependent, and may require clean positives and hard negatives that are not already available in labelled datasets.

% We address these challenges by introducing a unified tutor-move rubric and an online self-discovery preference training method for tutor-move steering. Our rubric integrates classic tutoring dialogue categories with feedback, funneling, focusing, and metacognitive support. Our training method generates candidate tutor turns under the current steering vectors, judges them using the tutor-move rubric and quality filters, and uses the resulting clean positives and hard negatives to update move-specific steering vectors.

% Our experiments show that the learned vectors steer LLM tutor responses toward targeted moves across held-out tutoring contexts and transfer to an unseen dataset. We also analyse steering-strength sensitivity, showing that some turns are easy to redirect while others remain resistant or become unstable only at high steering strengths. Finally, a user study evaluates whether controllable tutor moves affect perceived tutoring quality and student interaction.

% Our contributions are as follows:
% \begin{enumerate}
%     \item We introduce a unified tutor-move rubric for controllable LLM tutoring, combining classic tutoring dialogue acts with feedback, focusing, funnelling, and metacognitive support.
%     \item We propose an online self-discovery preference training method for tutor-move activation steering, where the model generates, judges, filters, and reuses its own tutor turns to learn move-specific steering vectors with dynamic hard-negative weighting and quality-filtered positives.
%     \item We evaluate tutor-move steering across validation, held-out, and unseen tutoring data, including steering-strength sensitivity and layer ablations.
%     \item We conduct a user study to assess whether controllable tutor moves improve perceived pedagogical quality and interaction experience.
% \end{enumerate}
